Robust Active Learning for More Efficient and Reliable Paths to Optimal Design

Simulation-driven design optimization requires active learning strategies that efficiently combine models with different computational costs and levels of fidelity. We introduce Multifidelity Cost-Aware Screening (MF-CAS), which enables the joint selection of sampling location and fidelity using a surrogate that provides decomposed uncertainty intervals rather than a complete predictive probability distribution. MF-CAS exploits the contribution of each fidelity to the high-fidelity uncertainty together with its computational cost to determine whether a candidate should first be evaluated at low fidelity or directly progressed towards high fidelity. The method is assessed on the constrained 14-dimensional hydrodynamic optimization of the DTMB 5415 hull under a deliberately limited computational budget. MF-CAS achieves an approximately 9.0% resistance reduction, compared with 6.7% for the best baseline optimisation method, demonstrating that incorporating fidelity-resolved uncertainty directly into the joint location-fidelity decision can substantially improve multifidelity active learning efficiency.

==> notation.tex <==
\usepackage{etoolbox} 
\usepackage[super,square,numbers]{natbib}

% ============================================================
% Mathematical notation
% ============================================================

% General notation
\newcommand{\DesignVector}{\ensuremath{\mathbf{x}}}
\newcommand{\DesignSpace}{\ensuremath{\mathcal{X}}}
\newcommand{\CandidateSet}{\ensuremath{\mathcal{X}_{\mathrm{cand}}}}
\newcommand{\PositivePart}[1]{\ensuremath{\left[#1\right]_{+}}}

\newcommand{\IterationIndex}{\ensuremath{k}}
\newcommand{\NextDesign}{\ensuremath{\mathbf{x}_{k+1}}}
\newcommand{\NextAction}{\ensuremath{a_{k+1}}}

% Fidelity labels
\newcommand{\LF}{\ensuremath{\mathrm{L}}}
\newcommand{\HF}{\ensuremath{\mathrm{H}}}
\newcommand{\LFHF}{\ensuremath{\mathrm{L{+}H}}}
\newcommand{\Correction}{\ensuremath{\delta}}

% Multifidelity datasets
\newcommand{\DataLF}{\ensuremath{\mathcal{D}_{\LF}}}
\newcommand{\DataHF}{\ensuremath{\mathcal{D}_{\HF}}}
\newcommand{\ObservedSitesLF}{\ensuremath{\mathcal{X}_{\LF}^{\mathrm{obs}}}}
\newcommand{\ObservedSitesHF}{\ensuremath{\mathcal{X}_{\HF}^{\mathrm{obs}}}}

% ------------------------------------------------------------
% Interface with the multifidelity surrogate
% ------------------------------------------------------------

% Predictive means
\newcommand{\MeanLF}[1]
{\ensuremath{\mu_{\LF}\!\left(#1\right)}}

\newcommand{\MeanCorrection}[1]
{\ensuremath{\mu_{\Correction}\!\left(#1\right)}}

\newcommand{\MeanHF}[1]
{\ensuremath{\mu_{\HF}\!\left(#1\right)}}

% Interpolation uncertainty
\newcommand{\InterpolationUncertaintyLF}[1]
{\ensuremath{U_{\mathrm{int},\LF}\!\left(#1\right)}}

\newcommand{\InterpolationUncertaintyCorrection}[1]
{\ensuremath{U_{\mathrm{int},\Correction}\!\left(#1\right)}}

% Training-point/data uncertainty
\newcommand{\DataUncertaintyLF}[1]
{\ensuremath{\sigma_{\LF}\!\left(#1\right)}}

\newcommand{\DataUncertaintyCorrection}[1]
{\ensuremath{\sigma_{\Correction}\!\left(#1\right)}}

\newcommand{\DataUncertaintyWeight}
{\ensuremath{\beta_{\sigma}}}

% Uncertainty contributions
\newcommand{\UncertaintyContributionLF}[1]
{\ensuremath{\omega_{\LF}\!\left(#1\right)}}

\newcommand{\UncertaintyContributionCorrection}[1]
{\ensuremath{\omega_{\Correction}\!\left(#1\right)}}

\newcommand{\UncertaintyHF}[1]
{\ensuremath{U_{\HF}\!\left(#1\right)}}

% ------------------------------------------------------------
% Active-learning quantities
% ------------------------------------------------------------

\newcommand{\BestObservedHF}
{\ensuremath{f_{\HF}^{\min}}}

\newcommand{\PredictedImprovementGap}[1]
{\ensuremath{d\!\left(#1\right)}}

\newcommand{\TotalPotential}[1]
{\ensuremath{P\!\left(#1\right)}}

\newcommand{\DeterministicPotential}[1]
{\ensuremath{D\!\left(#1\right)}}

\newcommand{\ExploratoryPotential}[1]
{\ensuremath{E\!\left(#1\right)}}

\newcommand{\ResidualUncertaintyHF}[1]
{\ensuremath{U_{\HF\setminus\LF}\!\left(#1\right)}}

\newcommand{\ResidualPotentialHF}[1]
{\ensuremath{P_{\HF\setminus\LF}\!\left(#1\right)}}

\newcommand{\ScreeningValueLF}[1]
{\ensuremath{S_{\LF}\!\left(#1\right)}}

\newcommand{\UncertaintyShareLF}[1]
{\ensuremath{\eta_{\LF}\!\left(#1\right)}}

\newcommand{\ImprovementValueLF}[1]
{\ensuremath{I_{\LF}\!\left(#1\right)}}

\newcommand{\RelativeUncertaintyLF}[1]
{\ensuremath{Q_{\LF}\!\left(#1\right)}}

% Action values
\newcommand{\ActionValueLF}[1]
{\ensuremath{V_{\LF}\!\left(#1\right)}}

\newcommand{\ActionValueHF}[1]
{\ensuremath{V_{\HF}\!\left(#1\right)}}

\newcommand{\ActionValueLFHF}[1]
{\ensuremath{V_{\LFHF}\!\left(#1\right)}}

% Costs and budget
\newcommand{\CostLF}{\ensuremath{c_{\LF}}}
\newcommand{\CostHF}{\ensuremath{c_{\HF}}}
\newcommand{\CostLFHF}{\ensuremath{c_{\LFHF}}}
\newcommand{\RemainingBudget}{\ensuremath{B}}

% Acquisition functions
\newcommand{\AcquisitionLF}[1]
{\ensuremath{\alpha_{\LF}\!\left(#1\right)}}

\newcommand{\AcquisitionHF}[1]
{\ensuremath{\alpha_{\HF}\!\left(#1\right)}}

\newcommand{\AcquisitionLFHF}[1]
{\ensuremath{\alpha_{\LFHF}\!\left(#1\right)}}

\newcommand{\AcquisitionAction}[2]
{\ensuremath{\alpha_{#1}\!\left(#2\right)}}

% Actions and admissible domains
\newcommand{\ActionSet}
{\ensuremath{\mathcal{A}}}

\newcommand{\AdmissibleDomainLF}
{\ensuremath{\mathcal{X}_{\LF}^{\mathrm{adm}}}}

\newcommand{\AdmissibleDomainHF}
{\ensuremath{\mathcal{X}_{\HF}^{\mathrm{adm}}}}

\newcommand{\AdmissibleDomainLFHF}
{\ensuremath{\mathcal{X}_{\LFHF}^{\mathrm{adm}}}}

\newcommand{\AdmissibleDomain}[1]
{\ensuremath{\mathcal{X}_{#1}^{\mathrm{adm}}}}

\begin{equation}
\PredictedImprovementGap{\DesignVector}=\BestObservedHF-\MeanHF{\DesignVector}, \qquad
\TotalPotential{\DesignVector}=\PositivePart{\PredictedImprovementGap{\DesignVector}+\UncertaintyHF{\DesignVector}},
\label{eq:HF_potential}
\end{equation}
